No Free Slide: Spurious Contact Forces in Incremental Potential Contact

Modeling contact between deformable solids is a fundamental problem in computer animation, mechanical design, and robotics. Existing methods based on $C^0$-discretizations -- piece-wise linear or polynomial surfaces -- suffer from discontinuities and irregularities in tangential contact forces, which can significantly affect simulation outcomes and even prevent convergence. To overcome this limitation, we employ smooth surface representations for both contacting bodies. Through a series of test cases, we show that our approach offers advantages over existing methods in terms of accuracy and robustness for both forward and inverse problems. The contributions of our work include identifying the limitations of existing methods, examining the advantages of smooth surface representation, and proposing forward and inverse problems to analyze contact force irregularities.

==> Method_backup.tex <==
\section{Deformable Contact Mechanics}
% We focus on solving the dynamics of deformable solids with contact in a frictionless setting. Given $n$ nodal positions $\bx$, finite-element lumped matrix $\bM$, an elastic energy $\Psi(\bx)$ and external force $\f_e$, we try to minimize the system energy
We focus on solving the dynamics of deformable solids with contact in a frictionless setting. Finding the dynamic force equilibrium configuration amounts to finding the minimum of the following potential
\begin{equation} \label{eq::dynamics}
   E(\bx) = \frac{1}{2} \dot\bx^{\tran} \bM \dot\bx + \Psi(\bx)e + \bx^{\tran} \f_e \ ,
\end{equation}
with geometrical constraints on contact surfaces. Here, $\bx$ denotes the nodal positions, $\bM$ is the mass matrix, $\Psi(\bx)$ is the elastic potential and $\bff_e$ is the external force.
Solving for the known position $\bx_{t+1}$ in the next time step using a fully implicit approach for time integration gives
% \begin{align}\label{eq::timestep}
% \begin{split}
%      \arg \min_{\bx} E(\bx) &= \frac{1}{2} \left(\frac{\bx-\bx_t}{h^2} -\frac{ \bv_t}{h}\right)^T \bM \left(\frac{\bx-\bx_t}{h^2} -\frac{ \bv_t}{h}\right) \\
%      &+ \Psi(\bx) + \bx^T \f_e \,
% \end{split}
% \end{align}
\begin{equation}
    \bx_{t+1} = \arg \min_{\bx} E(\bx) = \frac{1}{2h^2} (x^{\tran} \bM \bx - x^{\tran}\bM(\bx_t + \bv_th)) + \Psi(\bx) + \bx^{\tran} \f_e,
\end{equation}
where $h$ is the step size, $\bx_t$ and $\bv_t$ are the positions and velocities in the current time step $t$.
\paragraph{Contact Constraint} 
% For simplicity, we consider the deformable-to-deformable contact of a primary body $\mathcal{B}_1$ and a secondary body $\mathcal{B}_2$ in the continuous setting.
% The surfaces $\partial \mathcal{B}_i, i = 1,2$ are divided into three disjoint subsets $\Gamma^\sigma_i$, $\Gamma^u_i$
% and $\Gamma^c_i$, where $\Gamma^\sigma_i$, $\Gamma^u_i$ are the Neumann and Dirichlet boundaries, and $\Gamma^c_i$ is the potential contact surface. 
% Both bodies should satisfy the initial boundary value problem,
% \begin{equation} \label{eq::eq1}
% \begin{split}
%     \boldsymbol{b}_i + \nabla \boldsymbol{\sigma}_i = 0 \mbox{, for } \boldsymbol{x} \in \mathcal{B}_i \\
%     \boldsymbol{u}_i = \hat{ \boldsymbol{u}}_i \mbox{, for } \boldsymbol{x} \in \Gamma^u_i \\
%     \boldsymbol{\sigma}_i \cdot \boldsymbol{n} = \hat{\textbf{t}}_i \mbox{, for } \boldsymbol{x} \in \Gamma^\sigma_i,
% \end{split}
% \end{equation}
% where $\boldsymbol{b}_i, \boldsymbol{u}_i, \boldsymbol{\sigma}_i$ are prescribed body forces, tractions at Neumann boundaries displacements at Dirichlet boundaries, and $\boldsymbol{\sigma}_i, \boldsymbol{n}$ are the Cauchy stress tensor and unit normal vector at a point $\boldsymbol{x}$.
% When a deformable object is subject to external loads, its resulting deformation generates internal forces to balance the external forces. For the hyperelastic model we use, the internal forces are conservative and therefore can be expressed as the derivatives of the energy potential,
% \begin{equation} \label{eq::eq1}
%    \boldsymbol{f}^{int} (\boldsymbol{x}) = -\frac{\partial W^{int} (\boldsymbol{x})}{ \partial \boldsymbol{x}},
% \end{equation}
% where the energy potential is defined using an energy density $\Psi(\boldsymbol{F})$ integrated over the whole body as
% \begin{equation} \label{eq::eq2}
%     W^{int} (\boldsymbol{x}) = \int_{\mathcal{B}_i} \Psi(\boldsymbol{F}) d\mathcal{B}_i.
% \end{equation}
% The external forces $\boldsymbol{f}^{ext}(\boldsymbol{x})$ are prescribed on the Neumann boundaries $\Gamma^\sigma_i$. The deformable object reaches a quasi-static state if the force balance is achieved for all points of the body,
% \begin{equation} \label{eq::eq3}
%    \boldsymbol{f}^{int} (\boldsymbol{x})+\boldsymbol{f}^{ext} (\boldsymbol{x}) = \boldsymbol{0} \ , \boldsymbol{x} \in \mathcal{B}_i.
% \end{equation}
% If $\boldsymbol{f}^{ext}(\boldsymbol{x})$ is also conservative, solving the balance of force in Equation~(\ref{eq::eq3}) is equivalent to minimizing the total energy $W = W^{int}+W^{ext}$. To numerically compute the integral in Equation(\ref{eq::eq2}), we use a standard finite element method (FEM) that partitions the body $\mathcal{B}_i$ into subdomains and sum up the elastic energy for each subdomain.
The geometrical constraint between two deformable surfaces $\mathcal{B}_1$ and $\mathcal{B}_2$ is described through a measure for proximity known as the \textit{gap function} $g_n(\boldsymbol{x})$, which is defined as
\begin{equation} \label{eq::eq4}
    g_n(\boldsymbol{x}^{(1)}) = -\boldsymbol{n}_c\cdot(\boldsymbol{x}^{(1)}-\hat{\boldsymbol{x}}^{(2)}) \ ,
\end{equation}
where $\boldsymbol{x}^{(1)}$ denote points on $\mathcal{B}_1$, $\hat{\boldsymbol{x}}^{(2)}$ is the corresponding contact point on $\mathcal{B}_2$, and $\boldsymbol{n}_c$ is the normal vector. A standard choice for computing $\hat{\boldsymbol{x}}^{(2)}$ is based on the closest point projection, where
\begin{equation} \label{eq::eq5}
    \hat{\boldsymbol{x}}^{(2)} = \underset{\boldsymbol{x}^{(2)} \in \mathcal{B}_2}{\arg\min} \ ||\boldsymbol{x}^{(1)}-\boldsymbol{x}^{(2)}|| \ .
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The contact constraint requires the gap function to be non-negative for all $\bx^{(1)}_t$. This constraint can be formulated as a unilateral barrier function to impose strictly, 
\begin{align} \label{eq::log_barrier}
\begin{split}
     \phi(\bx^{(1)}_{i,t}) &= -(g_n(\bx^{(1)}_{i,t})-\hat{d})^2 \ln \left(\frac{g_n(\bx^{(1)}_{i,t})}{\hat{d}}\right) \ , \\
     & 0 < g_n(\bx^{(1)}_{i,t}) < \hat{d} \ .
\end{split}
\end{align}
%
% Given the gap function $g_n(\bx^{(1)}_{i,t})$, we have two options to enforce the non-negativity individually. 1. Use a cubic penalty that allows small penetration,
% \begin{equation} \label{eq::cubic_pen}
%     \phi(\bx^{(1)}_{i,t}) = - g_n(\bx^{(1)}_{i,t})^3 \ , \ g_n(\bx^{(1)}_{i,t}) < 0 \ .
% \end{equation}
% 2. Use a log-barrier potential that strictly enforces the constraints,
% \begin{align} \label{eq::log_barrier}
% \begin{split}
%      \phi(\bx^{(1)}_{i,t}) &= -(g_n(\bx^{(1)}_{i,t})-\hat{d})^2 \ln \left(\frac{g_n(\bx^{(1)}_{i,t})}{\hat{d}}\right) \ , \\
%      & 0 < g_n(\bx^{(1)}_{i,t}) < \hat{d} \ .
% \end{split}
% \end{align}

While this formulation is $C^2$-continuous as long as the gap function is continuous, maintaining this smooth property is challenging a piece-wise linear discretization due to the inherent discontinuity.
Although IPC-based methods manage to construct a smooth potential within this discrete setting, as we show in the following section, there is still a fundamental limitation rooted in the formulation.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% It's clear that a positive value of the gap function means the points are not in contact, while a negative value represents the penetration state. 
% The set of Karush-Kuhn-Tucker (KKT) conditions for frictionless contact on the contact surface can be described as
% \begin{equation} \label{eq::eq6}
%     g_n(\boldsymbol{x}) \geq 0 \mbox{, } p_n(\boldsymbol{x}) \leq 0 \mbox{, } g_n(\boldsymbol{x})p_n(\boldsymbol{x}) = 0,
% \end{equation}
% where $p_n(\boldsymbol{x})$ is the normal contact pressure. The first condition enforces the geometric constraints that the primary body cannot penetrate into the secondary body. The second condition implies no adhesive forces are allowed within the contact area. The last condition, known as the complementarity condition, requires the contact pressure exists only when the gap function is zero and the two bodies are in contact state. There are several standard solution techniques to approach the KKT conditions such as Lagrange multiplier methods or active set strategies. In our implementation, we choose the penalty method which results in additional contact energy to the total energy. The complementarity condition can also be approximated by either allowing a small penetration or using a barrier energy \cite{li2020incremental} that generates contact pressure when the gap function is small. In the following sections, we will discuss how contact energy is formulated.


%  Two-body contact problem in the continuous setting

%  Primary $\mathcal{B}_1$ and secondary $\mathcal{B}_2$ body.

%  Normal gap
% For each secondary point, we find closest point on primary surface. 
% Leads to minimization problem

% Then compute gap between those points.
 
\section{Contact Energy on Piecewise Linear Mesh}
Arguably one of the most standard ways of representing deformable surfaces is to use piecewise linear surface representation, especially when it comes to the use of the finite element method. 
%
However, maintaining the desired smoothness is particularly challenging in the discrete setting with piece-wise linear discretizations.
%
In this section, we first briefly review the Node-to-Segment method and explain why it fails to satisfy the smoothness requirement desired for optimization~\ref{sec:NTS}. We then discuss how the IPC approach successfully maintains $C^2$ continuity and the limitation at its costs.
\subsection{Node-to-Segment Method}
\label{sec:NTS}
% As discussed in the related works, methods for contact simulations can be classified into four types based on the primitives used in formulating the contact energies. The simplest approach, the pure node-based method, requires specific mesh discretization and is limited to small deformations. The STS method can be viewed as a precursor to the mortar method. In this section, we focus primarily on the NTS and mortar methods, including some of their extensions. We also provide a brief overview of the IPC formulation and its relation to the aforementioned categories. Despite its powerfulness, the IPC formulation can cause problems in a simple inverse design setting, which we discuss in detail.
% \begin{figure}[h]
%     \centering
%     \includegraphics[width = 0.4\textwidth]{imgs/nts_illustration.pdf}
%     \caption{Contact between two piecewise linear surfaces $\mathcal{B}_1$ and $\mathcal{B}_2$. Whereas the subscripts denote vertex index, the superscript indicates which surface it belongs to.}
%     \label{fig:ProblemIllustration}
% \end{figure}
Arguably one of the most standard ways of representing deformable surfaces is to use piecewise linear surface representation, especially when it comes to the use of the finite element method. 
%
However, maintaining the desired smoothness is particularly challenging in the discrete setting with piece-wise linear discretizations.
%
Fig.~\ref{fig:IssueWithNTSProjection} illustrates a scenario when two surfaces $\mathcal{B}_1$ and $\mathcal{B}_2$ are in closing contact and surface $\mathcal{B}_1$ is moving in the arrow direction.
%
To compute the \textit{gap} function for contact resolution, one has to first identify the contact primitive pairs and compute a distance measurement between the contact primitives.
%
Consider the one vertex on the surface $\mathcal{B}_1$ (shown in red), the closest edges on surface $\mathcal{B}_2$ change when it steps into or out from the shaded region (equal distance to both edges).
Consequently, the contact force experiences an abrupt change in direction, leading to only $C^0$ continuous across boundaries with discontinuous normals. 
\begin{figure}[h]
    \centering
    \includegraphics[width = 0.35\textwidth]{imgs/nts_illustration.jpg}
    \caption{Discontinuity across element boundary. As the red vertex moves in the arrow direction, stepping into or out of the gray region can lead to discontinuity in contact forces.}
    \label{fig:IssueWithNTSProjection}
\end{figure}
% In the context of a 2D scenario illustrated in Figure~\ref{fig:ProblemIllustration}, the enforcement of a geometrical constraint for a specific point (e.g., $\bx^{(1)}_3$) necessitates the specification of both the value of the gap function, denoted as $g_n(\bx^{(1)}_{3})$, and the points within $\mathcal{B}2$ that contribute to the calculation of $g_n(\bx^{(1)}_{3})$. This additional information is essential for accurately propagating the contact force. 
% %
% In the ensuing section, we delve into an examination of how the Node-to-Segment and Incremental Potential Contact approaches acquire such data, along with an exploration of potential issues associated with each methodology.



The NTS (Node-to-Segment) method is based on a straightforward concept: identifying the closest line segment and utilizing the distance between them as the value for the gap function. In the schematic example shown in Fig.~\ref{fig:IssueWithNTSProjection}, this involves projecting point $\bx^{(1)}_3$ onto line segment $\bx^{(2)}_3\bx^{(2)}_4$. If the resulting gap value is negative, it indicates the presence of a contact force attempting to separate them.

However, the NTS method suffers from a clear drawback inherent in its formulation. From an engineering standpoint, it oversimplifies the underlying physical model of the contact by placing virtual springs at each mesh vertex. Consequently, this approach leads to numerical inaccuracies, particularly when the mesh discretization is significantly imbalanced \cite{https://doi.org/10.1002/nme.2559}. Nonetheless, an even more critical issue arises when considering differentiability requirements. It is plausible for a single node to have equidistant distances to multiple line segments. For example in Figure~\ref{fig:IssueWithNTSProjection}, a point located in the gray shaded area will have the same closest distance to both segments  $\bx^{(2)}_2\bx^{(2)}_3$ and $\bx^{(2)}_3\bx^{(2)}_4$. While manually selecting one segment does not affect the computation of $g_n(\bx)$, such selection influences the contact force since only the chosen segment receives the force for $\bx$. Consequently, this introduces a discontinuity in the system.


% \begin{figure}[h]
%     \centering
%     \includegraphics[width = 0.45\textwidth]{imgs/fig1.png}
%     \caption{Element geometry of the Node-to-segment contact formulation. (Redraw later)}
%     \label{fig:shellCompBending}
% \end{figure}
% \textit{Classical Formulation}. Each contact element consists of a node $\boldsymbol{p}$ from the primary body and a segment $\boldsymbol S_1\boldsymbol S_2$ from the secondary body. The segment is chosen such that its closest distance to the node is minimized, which is the gap function $g_n(\boldsymbol{p})$. The contact energy for each element $W^{con}_{\boldsymbol{p}}$ is then defined as
% \begin{equation} \label{eq::eq7}
%     W^{con}_{\boldsymbol{p}} = \alpha \varepsilon_n g_n(\boldsymbol{p})_{-}^\beta,
% \end{equation}
% where $\alpha,\beta$ are suitably selected constants, $\varepsilon_n$ is the penalty parameter, and $g_n(\boldsymbol{p})_{-}$ means we take the minimum value between  $g_n(\boldsymbol{p})$ and $0$. In other words, we only consider the primary nodes that penetrate into the secondary body. In practice, we choose $\alpha = -1$ and $\beta = 3$. The total contact energy is then the summation of all the primary nodes
% \begin{equation} \label{eq::eq8}
%     W^{con} = \underset{\boldsymbol{x} \in \mathcal{B}_1} \sum W^{con}_{\boldsymbol{x}}.
% \end{equation}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width = 0.47\textwidth]{imgs/fig2.png}
%     \caption{Ambiguous closest point projection from one primary point to two secondary segments. (Redraw later)}
%     \label{fig:IssueWithNTSProjection}
% \end{figure}

% \textit{Limitations of the NTS Formulation.} There are two major problems with the NTS formulation that require further attention. First, the gap function calculation may pose difficulties when a primary node has the same distance to two secondary segments, as illustrated in Fig.~\ref{fig:IssueWithNTSProjection}. Such a scenario may disrupt the rate of convergence or even prevent convergence altogether \cite{ZAVARISE20093428}. Second, the force transmission from primary to secondary segments is overly simplified, being represented as nodal force transmission at discrete primary nodes. This approach, depicted in Fig.~\ref{fig:IssueWithNTSForceTransmission}, approximates a series of soft springs along the primary segments using a single, stiff spring at each primary node. Consequently, the resulting pressure distribution on the secondary surface is inaccurate, with some secondary segments experiencing more force than others.
% \begin{figure}[b]
%     \centering
%     \includegraphics[width = 0.47\textwidth]{imgs/fig3.png}
%     \includegraphics[width = 0.47\textwidth]{imgs/fig4.png}
%     \caption{Physical interpretation of the NTS formulation. (Redraw later)}
%     \label{fig:IssueWithNTSForceTransmission}
% \end{figure}

% \textit{Extensions.} Several extensions have been proposed to address the aforementioned issues with the classical NTS formulation \cite{https://doi.org/10.1002/nme.2559}. The crux of the matter is to make the penalty parameter $\varepsilon_n$ dependent on the reference geometry rather than a constant. As depicted in Fig.~\ref{fig:IssueWithNTSForceTransmission}, at point $\boldsymbol{S}$, $\varepsilon_n$ is proportional to the length $l_{AS}+l_{SB}$, where primary segments $AS$ and $SB$ together constitute the \textit{area of competence} of point $\boldsymbol{S}$. However, this extension alone is insufficient. Even if a primary node can now accurately transmit the force within its area of competence, only one secondary segment can receive that force. Consequently, if such an area encompasses more than one secondary segment, one segment will receive more force than it should, while all other segments will receive no contribution from that primary node. One way to address this issue is to use \textit{virtual} nodes instead of mesh vertices when computing the contact energy such that the area of competence of each virtual node projects onto only one secondary segment. However, this approach may require recomputation of virtual node locations as the two bodies deform, which can be computationally expensive at the outset.

% \subsection{Mortar Method}
% The physical interpretation of the NTS formulation suggests that the most effective approach to computing contact energy is to calculate the contributions of the "small springs" directly along the primary segments. This principle forms the basis of the mortar method, which involves dividing the primary and secondary surfaces into mortar segments, quadrilaterals comprising two points on each surface. The contact energy can be computed by integrating it over each of these segments, as shown in the following equation,
% \begin{equation} \label{eq::eq9}
%     W^{con} = \underset{\boldsymbol{m} \in \mathcal{M}} \sum W^{con}_{\boldsymbol{m}},
% \end{equation}
% where $m$ represents one mortar segment and $\mathcal{M}$ is the set of all segments on the potential contact surface.

% \begin{figure}[b]
%     \centering
%     \includegraphics[width = 0.4\textwidth]{imgs/fig5.png}
%     \includegraphics[width = 0.4\textwidth]{imgs/fig6.png}
%     \caption{Two ways of partitioning the mortar segments. (Redraw later)}
%     \label{fig:MortarSegments}
% \end{figure}

% \textit{Partitioning Mortar Segments.} The most intuitive way to find the mortar segments is through the projection of the nodes from one surface to another as depicted in Fig.~\ref{fig:MortarSegments}. However, this partition encounters the same projection ambiguity in Fig.~\ref{fig:IssueWithNTSProjection}. To address this issue, Yang et al. \shortcite{https://doi.org/10.1002/nme.1222} proposed a novel segmentation method based on the concept of \textit{continuous normal field}. This method involves calculating the normal at each mesh vertex as the weighted average of its adjacent segments and defining the normal within one segment as a linear interpolation between the normals at its endpoints. By utilizing the continuous normal, the projection from the primary surface to the secondary surface can be directly computed, while the projection from a secondary point to the primary surface can be attained by finding a point on the primary surface such that the line connecting them aligns with the normal at that point. Such projection is always unique because a ray can only intersect a piecewise linear curve once and the mortar segment is well-defined.

% \textit{Evaluation of Contact Energy per Segment.} Consider a mortar segment in Fig.~\ref{fig:IssueWithNTSProjection} with primary points $\boldsymbol\xi^a_1,\boldsymbol\xi^b_1$ and secondary points $\boldsymbol\xi^a_2,\boldsymbol\xi^b_2$. Any primary points on line segment $\boldsymbol\xi^a_1 \boldsymbol\xi^b_1$ can be parameterized using local coordinate $\eta \in [-1,1]$ as $\boldsymbol\xi_1(\eta)$. With the continuous normal field, we can compute its projected secondary point $\boldsymbol \Pi_2(\boldsymbol\xi_1(\eta))$ using the normal $\boldsymbol n_1(\eta)$ at $\boldsymbol\xi_1(\eta)$. The gap value is then calculated using the following equation,
% \begin{equation} \label{eq::eq10}
%     g_n(\boldsymbol\xi_1(\eta)) = - \boldsymbol n_1(\eta) \cdot [ \boldsymbol \xi_1(\eta) - \Pi_2(\boldsymbol \xi_1(\eta)) ].
% \end{equation}
% The integral of the contact energy within the mortar segment can be expressed as
% \begin{equation} \label{eq::eq11}
%    W^{con}_{\boldsymbol{m}} = \int^1_{-1} \alpha \varepsilon_n g_n^\beta(\eta)_{-} J_{\eta} d\eta,
% \end{equation}
% where we need the Jacobian $J_{\eta}$ since we change from global coordinate to local coordinate. In practice, equation (\ref{eq::eq11}) is evaluated using Gaussian quadrature.

% \textit{Discussion.} The mortar method is a prevalent technique in engineering to address contact problems due to its high numerical accuracy. However, this method has several limitations that constrain its wider adoption. Firstly, the method is more intricate than the NTS method, requiring multiple projections even when computing energy for a single segment. Secondly, extending the algorithm to 3D necessitates remeshing, as the projected secondary points often lie within a primary triangular face, leading to undesired discontinuities when considering inverse design. Despite these drawbacks, the concept of continuous normal fields has inspired the use of implicit surface representation in formulating contact energy, as elaborated in the subsequent section.

\subsection{Incremental Potential Contact}
\label{sec:NTS}
% In the last part of this section, we provide a succinct overview of the formulation of contact energy within the domain of IPC, a cutting-edge computational approach utilized for simulating an array of materials in computer graphics. Specifically, our emphasis is centered on the methodology employed by IPC for enforcing non-penetration constraints, as well as computing the separation distance between interacting objects. Furthermore, we delineate a scenario in which IPC is susceptible to failure, and explicate the underlying cause. This failure scenario serves as an additional impetus for our IMLS contact method.

% \textit{Nonpenetration Enforcement and Distance Computation.} 
IPC relies on a barrier-augmented incremental potential to enforce non-intersection conditions between close primitive pairs, \eg, vertex-triangle, and edge-edge pairs. This involves finding a constraint set comprising primitives in close proximity. 
Whereas the NTS method selects for each vertex the closest segment, IPC allows multiple contact pairs for the same vertices to be active simultaneously. The collision response for any given vertex is given as the superposition of per-primitive potentials, which are modeled using uses smoothly-clamped, locally-supported barrier functions. Removing the need to make discrete decisions eliminates an important source of non-smoothness. However, the superposition principle also induces energy variations when multiple per-primitives become active. 
%
Subsequently, a smoothly clamped barrier energy is computed, which generates a local repulsive force to disentangle the primitives, provided that the distance between them is smaller than a specified threshold. One constituent of the constraint set comprises a point and a triangle or two edges, and the distance can be calculated via a constrained optimization problem, which has a closed-form solution in the majority of cases. The enforcement of $C^2$ continuity for the distance function necessitates special treatment solely in the case of contact between edges that are nearly parallel.

\subsection{Spurious Tangential Forces in IPC}
\begin{figure}[h]
    \centering
    \includegraphics[width = 0.5\textwidth]{imgs/EnergyWallEx.jpg}
    \includegraphics[width = 0.4\textwidth]{imgs/fig8.png}
    \caption{A simple test shows irregularities in IPC's contact potential. A single vertex is moved at constant distance to a triangulated plane and the contact energy is plotted. Near edges and vertices, multiple per-primitive potentials are active, leading to energy wall, i.e., local maxima in contact energy whose gradients resist tangential motion. }
    \label{fig:IPCEnergyWall}
\end{figure}


IPC and the NTS method share a similar approximation approach in that the gap between two contact surfaces is evaluated as the pointwise distance in the constraint set.  However, IPC avoids ambiguities in closest-point projection by considering multiple active collisions primitives for a given vertex Fig.~\ref{fig:IssueWithNTSProjection}. The corresponding contact energy for point $\bx^{(1)}_{3}$ is computed as 
\begin{equation}
    E_{IPC} = \kappa \sum_{i \in C} E_i =\kappa ( \phi(\bx^{(1)}_{3}, \bx^{(2)}_{2}\bx^{(2)}_{3}) + \phi(\bx^{(1)}_{3}, \bx^{(2)}_{3}\bx^{(2)}_{4}))
\end{equation}
In this way, IPC preserves continuity and differentiability in energy calculation. 

Unfortunately, the superposition of per-primitive potentials lead to undesirable \textit{energy walls} when a vertex is close to several triangles. Here we illustrate this using a simple setting (Fig.\ref{fig:IPCEnergyWall}), where we consider the IPC energy between a vertex $v$ and a rectangle with an initial distance smaller than the barrier threshold. As $v$ moves towards the right-hand side, the constraint set progresses from having one element (from $v$ to face $\bx_1\bx_2\bx_4$) to three elements (from $v$ to faces $\bx_1\bx_2\bx_4$, $\bx_2\bx_5\bx_4$, and $\bx_2\bx_3\bx_5$) to two elements (from $v$ to faces $\bx_2\bx_3\bx_5$ and $\bx_3\bx_6\bx_5$), as evidenced in the energy plot in Fig.~\ref{fig:IPCEnergyWall}. These energy walls give rise to spurious tangential forces that affect equilibrium states and they may impede progress in optimization when solving inverse problems. We elaborate further on this issue in Sec. \ref{sec:analysis}.

% https://epubs.siam.org/doi/epdf/10.1137/110848190
\section{IMLS}
We attribute the aforementioned issues of the NTS and the IPC methods to geometrical representation. 
If we are able to construct a smooth surface from the mesh and evaluate its distance to a given point, we can remove the ambiguity in orthogonal projection or duplication of closest primitives. The \textit{Implicit Moving-Least Squares} surface provides an efficient tool to evaluate the signed distance function. In this section, we present an augmentation to the NTS method using IMLS surface to create a fully differentiable and physically sensible contact energy formulation.

\subsection{Basics}
% Describe IMLS interpolation
Given $n$ points $\boldsymbol{x}_i \in \mathbb{R}^d$ and their normals $\boldsymbol{n}_i$, Kolluri \shortcite{kolluri2008provably} formulated an implicit formula $f(\boldsymbol{x})$ to describe a reconstructed surface from the point cloud,
\begin{equation} \label{eq::eq12}
  f(\boldsymbol{x}) = \frac{\sum \boldsymbol{n}^T_i (\boldsymbol{x}-\boldsymbol{x}_i)\boldsymbol{\phi}_i(\boldsymbol{x})}{\sum \boldsymbol{\phi}_i(\boldsymbol{x})},
\end{equation}
where $\boldsymbol{\phi}_i(\boldsymbol{x})$ is a symmetric weighted function that assigns more weight to sample points near $\boldsymbol{x}$. 

By definition, such formulation only works for smooth surfaces, which results in over-smoothing or instability on sharp features. Oztireli et al. \shortcite{oztireli2009feature} proposed an augmentation to the IMLS formulation to preserve features around sharp corners using the idea of \textit{robust local kernel regression}, where outliers are given less weight. The implicit surface is now defined by a Iteratively Reweighted Least Squares (IRLS) minimization,
\begin{equation} \label{eq::eq13}
  f^k(\boldsymbol{x}) = \underset{s_0}{\arg\min} \sum (s_0+(\boldsymbol{x}_i-\boldsymbol{x}^T)\boldsymbol{n}_i)^2\phi_i(\boldsymbol{x}) w(r^{k-1}_i),
\end{equation}
where $r^{k-1}_i$ is the residual $f^{k-1}(\boldsymbol{x}) - (\boldsymbol{x}_i-\boldsymbol{x})^T \boldsymbol{n}_i$. Oztireli et al. also observed that the samples belonging to different surface patches across a discontinuity should not be interpreted as outliers, while their normals should. This observation inspires the use of a new re-weighting term $w_n$ that penalizes the samples that have normals far away from the reconstructed IMLS surface. The final Robust IMLS surface now becomes
\begin{equation} \label{eq::eq14}
  f^k(\boldsymbol{x}) = \frac{\sum (s_0+(\boldsymbol{x}_i-\boldsymbol{x}^T)\boldsymbol{n}_i)^2\phi_i(\boldsymbol{x}) w(r^{k-1}_i) w_n(\Delta\boldsymbol{n}_i^{k-1})}{\sum \phi_i(\boldsymbol{x}) w(r^{k-1}_i) w_n(\Delta\boldsymbol{n}_i^{k-1})} ,
\end{equation}
where $\Delta\boldsymbol{n}_i^{k-1} = ||\nabla f^k(\boldsymbol{x})-\boldsymbol{n}_i||$ is the measure of a sample normal $\boldsymbol{n}_i$ and the predicted normal at query point $\boldsymbol{x}$. We use $\psi(\boldsymbol{x})$ instead of $f^k(\boldsymbol{x})$ to represent the signed distance function for convenience in the subsequent literature.



\subsection{Mesh to IMLS}
We augment the NTS method by first introducing a mesh vertex to IMLS surface formulation, wherein the IMLS surface is constructed based on the mesh vertices of the secondary object. Calculation of per-vertex normals is essential for this construction, which is accomplished using a method similar to the continuous normal field described in the Mortar method. Here, the normal of a mesh vertex is obtained as a weighted average of the edge (face) normals of its adjacent edges (faces). The gap value $g_n(\boldsymbol{p})$ in equation (\ref{eq::eq7}) is then substituted with the signed distance function $\psi(\boldsymbol{p})$ in equation (\ref{eq::eq14}), allowing for the easy integration of extensions such as area augmentation or virtual nodes in the NTS method without requiring additional changes in the code.

Using IMLS surfaces, it becomes unnecessary to locate the closest segment to a given point, thus eliminating any ambiguity that may arise. Moreover, the contact energy is now independent of the mesh topology, which implies that no energy walls are present while a point moves along a smooth surface as IPC. Finally, Levin \shortcite{levin1998approximation} has demonstrated that the signed distance function $f(\boldsymbol{x})$ of an IMLS surface is continuously differentiable when the weighting terms $\phi(\boldsymbol{x})$ are continuously differentiable. Hence, the energy formulation presented in this study is entirely differentiable if we choose suitable weight terms for $\phi$, $w$, and $w_n$.

\subsection{IMLS to IMLS}
We further extend the idea of computing the gap between a mesh vertex and an IMLS surface to computing the gap distance directly between two IMLS surfaces. However, we cannot get rid of the mesh vertices as they are needed for elastic energy computation. Consequently, we still use them as a guide to finding points on the IMLS surfaces. Given a point $\boldsymbol{x}_i$ on the primary mesh, its closest projection on the primary IMLS surface is $\boldsymbol{x}_i^1$. The distance between $\boldsymbol{x}_i^1$ and the secondary surface is directly given by $\psi_2(\boldsymbol{x}_i^1)$. The constrained optimization problem for finding the equilibrium state can be written as
\begin{equation} \label{eq::eq15}
\begin{aligned}
 \underset{\boldsymbol{x}}{\min} \quad & W^{int}(\boldsymbol{x}) + W^{ext}(\boldsymbol{x}) + W^{con}(\boldsymbol{x}^1) \\
 \textrm{s.t.} \quad & \boldsymbol{x}^1 = \underset{\boldsymbol{y}, \boldsymbol \psi_2(\boldsymbol y) = \boldsymbol 0}{\arg\min} ||\boldsymbol x- \boldsymbol{y}||^2_2.
 \end{aligned}
\end{equation}

In practice, we treat $\boldsymbol{x}^1$ as additional degrees of freedom and convert the constraints in equation (\ref{eq::eq15}) as additional penalty terms, that is,
\begin{equation} \label{eq::eq16}
\begin{aligned}
 \underset{\boldsymbol{x}}{\min} \quad & W^{int}(\boldsymbol{x}) + W^{ext}(\boldsymbol{x}) + W^{con}(\boldsymbol{x}^1) \\
 &+ \lambda_1 ||\boldsymbol x- \boldsymbol{x}^1||^2_2 + \lambda_2 \boldsymbol \psi_2(\boldsymbol x^1)^2.
 \end{aligned}
\end{equation}
This unconstrained optimization problem can be solved using Newton's method.


Let $\bx^1$ and $\bx^2$ denote the vertices of the first and second surface, respectively. 
In the continuous setting, we would like to ensure that each point on surface one has a positive distance to surface 2. In the discrete setting, we enforce this condition on a number of sample points distributed across the surfaces. These sample points should be distributed evenly across the surface, and they must lie on the surface. In our prototype implementation, we simply place a contact sample point at each vertex of the triangle mesh defining the IMLS surface, but other options such as triangle barycenters are of course possible.
Since contact sample points are not automatically on the surface, we have to ensure this condition through additional constraints, i.e., $\Psi_2(\bq^1_i)=0\ \forall i$ and likewise for $\Psi_1(\bq^2_i)=0\ \forall i$. 





==> _Results.tex <==
\section{Result} 
\label{sec:analysis}
\section{Comparison with IPC}
\paragraph{Qualitative comparison.}
We compare our approach with IPC on a simple example of a sliding cube on a plane in a frictionless section. As can be seen from 
\paragraph{Quantitative comparison.}

In this section, we conduct various numerical experiments to evaluate the performance of the aforementioned contact methods in comparison to our proposed IMLS-based contact formulation. 
%
Although our main focus in this section is on presenting the numerical results, we also consider the implementation and computational complexity of the methods. A comprehensive summary of these aspects is provided in Table~\ref{table:Comparisons}.

\begin{table}[b]
\begin{center}
\begin{tabular}{||c c c c c||} 
 \hline
 Criteria & NTS & Mortar & IPC & IMLS \\ [0.5ex] 
 \hline\hline
 Numerical Accuracy & - & +++ & + & ++ \\ 
 \hline
 Implementation Complexity & +++ & - & ++ & ++\\
 \hline
 Continuity \& Differentiability & + & + & - & +++\\
 \hline
 Computational Complexity & +++ & - & + & + \\
 \hline
\end{tabular}
\caption{Comparison results of the four contact-solving methods.}
\label{table:Comparisons}
\end{center}
\end{table}

\subsection{Numerical Experiments}
An overview of the numerical experiments is presented here. We select the tests with simple settings and known numerical ground truths while reflecting major differences among the methods.

% \paragraph{Contact Patch Test}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width = 0.45\textwidth]{imgs/p12.png}
%     \caption{Contact Patch Test Setting}
%     \label{fig:ContactPatchTestSetting}
% \end{figure}
% The contact patch test was initially introduced by Taylor et al.\shortcite{taylor1991patch} as a means of verifying whether a contact formulation can effectively transmit the appropriate normal stresses between two contact surfaces, independent of their discretization. In our experiment, we conducted the test depicted in Fig. \ref{fig:ContactPatchTestSetting}, wherein nodal forces were applied to the upper block to maintain a constant pressure on its contact surface. A proper contact formulation would then convey uniform normal stresses from the upper block to the lower one. As such, we were able to assess the precision of each method based on the nodal forces on the contact surface in the state of equilibrium.

% \paragraph{Normal Contact Test}
% \begin{figure}[b]
%     \centering
%     \includegraphics[width = 0.18\textwidth]{imgs/p14.png}
%     \caption{Normal Contact Test Setting}
%     \label{fig:NormalContactTestSetting}
% \end{figure}
% To conduct a more comprehensive evaluation of the numerical precision of each method, we perform a normal contact test on two curved surfaces. The pressure distribution between two elastic balls in Fig. \ref{fig:NormalContactTestSetting} can be computed using Hertz's classical theory, assuming the strain is small compared to the dimension of objects. Additional information regarding the analytical solution can be found in Appendix A. Moreover, we run the test at varying resolutions to assess the convergence of each method under refinement.

\paragraph{Sliding Test}
\begin{figure}[h]
    \centering
    %\includegraphics[width = 0.35\textwidth]{imgs/p18.png}
    \includegraphics[width = 0.30\textwidth]{imgs/sliding.png}
    \caption{Sliding Test Setting}
    \label{fig:SlidingContactTestSetting}
\end{figure}
The final numerical test we conducted provides a practical example wherein the energy walls depicted in Fig. \ref{fig:IPCEnergyWall} result in the failure of an inverse problem, while our IMLS contact is capable of achieving the intended design objective. The test configuration is illustrated in Fig. \ref{fig:SlidingContactTestSetting}, where we place points $A,B$ on two circular tracks with different radius and connect them with a virtual spring. If we move $B$ smoothly along the track (to $B'$), A will move accordingly (to $A'$) in its equilibrium state. The inverse problem entails determining the initial position $B$ such that $A$ will rest on a given target angle $\theta$.

% where an elastic block is positioned atop a rigid block and deforms when subjected to applied forces on top. When smoothly sliding the elastic block on the rigid surface, the right boundary of the elastic block in the state of equilibrium should likewise slide smoothly. The inverse problem entails determining the initial position of the elastic block based on the rest position of its right boundary $B$.

% Might not be the same for all experiments. Mortar for 2D contact patch. For 3D?
% What happens under refinement for all methods?
% Are there analytical solutions?

% \subsubsection{Contact Patch Test}
% \begin{figure}[b]
%     \centering
%     \includegraphics[width = 0.45\textwidth]{imgs/fig9.png}
%     \caption{Results of the Contact Patch Test}
%     \label{fig:ContactPatchTestResult}
% \end{figure}
% As previously mentioned, the mesh depicted in Fig. \ref{fig:ContactPatchTestSetting} is subjected to normal nodal forces, where the edges on the upper boundary of the primary block are uniformly pressured at the ratios of $F_1:F_2:F_3:F_4:F_5 = 1:2:3:4:2$. Ideally, the contact surfaces should have uniform pressure, and the forces applied to the secondary block should follow the ratio of $3:6:7:6:2$. The relative error at the secondary contact nodes is computed for each method and presented in Fig. \ref{fig:ContactPatchTestResult}. The results for the original NTS method are not included due to its significantly larger error of around 20\% compared to the other methods.

% From the results shown in Fig. \ref{fig:ContactPatchTestResult}, it is evident that the Mortar method exhibits the best performance with almost zero error. The IPC and our IMLS-to-IMLS formulation demonstrate slightly inferior performance at the boundary. The error in the IPC method is attributed to the "energy walls," as the primary and secondary contact nodes match only at the left or right boundary. Despite utilizing a robust IMLS formulation to preserve sharp features, it still fails to represent perfect squared corners and causes numerical errors in those regions. Our vanilla Vertex-to-IMLS formulation exhibits similar performance to the NTS method with virtual nodes and area augmentation, with the former being slightly superior because the forces are transmitted only to the node's closest segment in NTS formulation, whereas constructing the IMLS surface involves all nearby points.

% \subsubsection{Normal Contact Test}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width = 0.45\textwidth]{imgs/NormalTestR1.png}
%     \includegraphics[width = 0.45\textwidth]{imgs/NormalTestR2.png}
%     \caption{Results of the Normal Patch Test}
%     \label{fig:NormalPatchTestResult}
% \end{figure}
% In the second test scenario, we compare the performance of different contact methods on curved surfaces as depicted in Fig.\ref{fig:NormalContactTestSetting}. We calculate the nodal pressure at the contact surface and compare it with the analytical solution. We perform the test on the same geometry with different resolutions on the contact surfaces. The result is summarized in Fig.\ref{fig:NormalPatchTestResult} where we use Vertex-to-IMLS formulation for higher efficiency.

% While the three methods are all relatively close to the ground truth, IPC generates spikes near the center, which still exist even when we increase the resolutions. We again attribute this to the energy walls as the mesh vertex matches at the central point. Meanwhile, choosing the barrier distance is also crucial for IPC in this test, as a large weight may introduce an over-exaggeration of the gap, while a small value will cause a convergence issue.

% The Mortar method exhibits the best numerical accuracy in the lower-resolution test, but it suffers from huge computational complexity when we move to the higher-resolution case. The time for building the contact hessian is less than 0.1 seconds for IPC and around 5 seconds for our IMLS method and it takes more than 250 seconds for the mortar method to complete the same task. Our IMLS method strikes a balance between accuracy and efficiency and improves under refinement.

\subsubsection{Sliding Test}
\begin{figure}[ht]
    \centering
    \includegraphics[width = 0.45\textwidth]{imgs/Contactenergy.png}
    \includegraphics[width = 0.45\textwidth]{imgs/InverseDesign.png}
    \caption{Results of the Sliding Test}
    \label{fig:SlidingTestResult}
\end{figure}
% In the third numerical test, we design a simple inverse problem that the IPC method could fail on. Suppose $A$ lies on the track with radius $r_1$ and $B$ lies on the track with radius $r_2$. We want to determine the initial position of $B = (r_2\cos(\theta_p),-r_2\sin(\theta_p))$ such that $A$ will rest on $(r_1\cos(\theta_t),-r_1\sin(\theta_t))$ in its equilibrium state. This can be formulated as an optimization problem with the objective function $O(\theta_p) = \frac{1}{2}\lambda(\theta(\theta_p) - \theta_t)^2$ and further solved using sensitivity analysis.

% We observe that for target angles $\theta_t$ whose corresponding position on the track is close to some mesh vertex (for example $\theta_t = 0.2001$ in Fig.\ref{fig:SlidingContactTestSetting}), the optimization problem cannot converge to find $\theta_p$ while NTS and our IMLS formulation can. To explain the reason, we plot the contact energy as we move $A$ along the track and the result is shown in Fig.\ref{fig:SlidingContactTestSetting}, where the IPC method generates several energy walls with twice the value as the base one. The virtual spring is therefore difficult to "drag" $A$ across such walls and fail to give the correct rest positions. We also observe that the energy is not completely constant for our IMLS method. This is because the reconstructed IMLS surface is not perfect at the sharp energy and can be improved under mesh refinement or more optimization iterations as in equation(\ref{eq::eq14}). However, we can not make the energy wall decrease simply by increasing the mesh resolution.

In the third numerical test, we present a simple inverse problem that highlights a limitation of the IPC method. Specifically, we aim to determine the initial position of point $B$ on a track of radius $r_2$ such that point $A$ at rest on a track of radius $r_1$ in its equilibrium state coincides with a given target point on the track. To this end, we formulate an optimization problem with an objective function and solve it using sensitivity analysis. 

We observe that the IPC method fails to converge when the target point is located near a mesh vertex due to the presence of energy walls, as illustrated in Fig.\ref{fig:SlidingContactTestSetting}. Notably, the IPC method generates energy walls with twice the value of the base energy, making it difficult for the virtual spring to overcome the barrier and converge to the correct solution. In contrast, our NTS and IMLS methods can accurately solve the problem. We also note that although the energy is not entirely constant for the IMLS method, it can be improved by mesh refinement or additional optimization iterations. However, increasing the mesh resolution alone cannot mitigate the effect of energy walls.

\subsection{Qualitative Experiments}
To complete the analysis of IPC and our IMLS contact method, we also present several qualitative results that show the limitation of IPC with their original code as well as the ability of our IMLS method in complex 3D scenes.

\subsubsection{Limitation of IPC}
\begin{figure*}[h]
    \centering
    \includegraphics[width = 1.0 \linewidth]{imgs/IPC_fail.pdf}
    \caption{Demonstration of IPC failure in a simple scenario.
    }
    \label{fig:ipc_failure}
\end{figure*}
We reproduce the spurious tangential forces using the original code from Li et al.\shortcite{Li2020} under a simple setting illustrated in Figure~\ref{fig:ipc_failure}. We put a cube on a triangular mesh and exert a lateral force to move it to the right. We observe that even if we set the frictional coefficient to zero, the cube will stop once it touches an edge of the triangular mesh as if there is a wall stopping it. This spurious force will not disappear by simply decreasing the barrier distance $\hat{d}$. Please refer to the supplemental video for more examples.

\subsubsection{IMLS in 3D}


